Discriminated Belief Propagation

Near optimal decoding of good error control codes is generally a difficult task. However, for a certain type of (sufficiently) good codes an efficient decoding algorithm with near optimal performance exists. These codes are defined via a combination of constituent codes with low complexity trellis representations. Their decoding algorithm is an instance of (loopy) belief propagation and is based on an iterative transfer of constituent beliefs. The beliefs are thereby given by the symbol probabilities computed in the constituent trellises. Even though weak constituent codes are employed close to optimal performance is obtained, i.e., the encoder/decoder pair (almost) achieves the information theoretic capacity. However, (loopy) belief propagation only performs well for a rather specific set of codes, which limits its applicability. In this paper a generalisation of iterative decoding is presented. It is proposed to transfer more values than just the constituent beliefs. This is achieved by the transfer of beliefs obtained by independently investigating parts of the code space. This leads to the concept of discriminators, which are used to improve the decoder resolution within certain areas and defines discriminated symbol beliefs. It is shown that these beliefs approximate the overall symbol probabilities. This leads to an iteration rule that (below channel capacity) typically only admits the solution of the overall decoding problem. Via a Gauss approximation a low complexity version of this algorithm is derived. Moreover, the approach may then be applied to a wide range of channel maps without significant complexity increase.

==> TR-gloss.tex <==

\subsection{Glossary}

\begin{tabular}{ll}
$\left\langle b\right\rangle $ & Map of Boolean to $\{0,1\}$ given by $0$ if $b$ false and 1 if
$b$ true.\tabularnewline
\noalign{\vskip2pt}
$\mathbb{A}$ & Shorthand for the set $\mathbb{E}(A)$.\tabularnewline
\noalign{\vskip2pt}
$\mathbb{A}_{n\varepsilon}(\mathbf{C}|\mathbf{r})$ & Typical set given by $\{\mathbf{c}:|H(\mathbf{c}|\mathbf{r})-H(\mathbf{C}|\mathbf{r})|\leq n\varepsilon\}$
and $\mathbf{c}\in\mathbb{C}$.\tabularnewline
\noalign{\vskip2pt}
$\mathbb{A}_{n\varepsilon}(\mathbf{S}|\mathbf{w})$ & Typical set given by $\{\mathbf{s}:|H(\mathbf{s}|\mathbf{w})-H(\mathbf{S}|\mathbf{w})|\leq n\varepsilon\}$
and $\mathbf{s}\in\mathbb{S}$.\tabularnewline
\noalign{\vskip2pt}
$\mathbb{A}_{n\varepsilon}(\mathbf{S}|\mathbf{w}\Vert\mathbf{r})$ & Cross typical set given by \tabularnewline
\noalign{\vskip2pt}
 & ~~$\{s:\min(H(\mathbf{S}|\mathbf{w}),H(\mathbf{C}|\mathbf{w}\Vert\mathbf{r}))-n\varepsilon\leq H(\mathbf{s}|\mathbf{w})\leq\max(H(\mathbf{S}|\mathbf{w}),H(\mathbf{C}|\mathbf{w}\Vert\mathbf{r}))+n\varepsilon\}.$\tabularnewline
\noalign{\vskip2pt}
$\mathbb{B}$ & Set $\{-1,+1\}$.\tabularnewline
\noalign{\vskip2pt}
$\hat{\mathbf{c}}^{(a)}$ & ML decision of the overall code.\tabularnewline
\noalign{\vskip2pt}
$\bar{c}_{i}^{(a)}$ & ML decision of the binary symbol $C_{i}$ of the overall code.\tabularnewline
\noalign{\vskip2pt}
$\mathbf{C}$ & General code.\tabularnewline
\noalign{\vskip2pt}
$\mathbf{C}^{(a)}$ & Overall code with code words $\mathbf{c}^{(a)}=(c_{1}^{(a)},\ldots,c_{n}^{(a)})$.\tabularnewline
\noalign{\vskip2pt}
$\mathbf{C}^{(l)}$ & Constituent code with code words $\mathbf{c}^{(l)}=(c_{1}^{(l)},\ldots,c_{n}^{(l)})$.\tabularnewline
\noalign{\vskip2pt}
$\mathbb{C}=\mathbb{E}(\mathbf{C})$ & Set of the code words of a general code.\tabularnewline
\noalign{\vskip2pt}
$d_{H}(\mathbf{c},\mathbf{r})$ & \noun{Hamming} distance given by $\sum_{i=1}^{n}\left\langle c_{i}=r_{i}\right\rangle $.\tabularnewline
\noalign{\vskip2pt}
$\mathbb{E}(A)$ & Event set of the random variable $A$.\tabularnewline
\noalign{\vskip2pt}
$\mathrm{E}[f(a)|b]$ & Expectation of $f(a)$ under $b$ given by $\mathrm{E}_{A|B}[f(a)|b]=\sum_{b\in\mathbb{E}(B)}f(a)P(a|b)$.\tabularnewline
\noalign{\vskip2pt}
$\mbox{exp}_{2}(x)$ & Binary exponent given by $2^{x}$.\tabularnewline
\noalign{\vskip2pt}
$H(\mathbf{C}|\mathbf{r})$ & Entropy of $\mathbf{C}$ under $\mathbf{r}$ given by $\mathrm{E}_{\mathbf{C}}[H(\mathbf{c}|\mathbf{r})|\mathbf{r}]$
and $H(\mathbf{c}|\mathbf{r})=-\log_{2}(P(\mathbf{c}|\mathbf{r}))$.\tabularnewline
\noalign{\vskip2pt}
$H(\mathbf{S}|\mathbf{r})$ & Entropy of $\mathbf{S}$ under $\mathbf{r}$ given by $\mathrm{E}[H(\mathbf{s}|\mathbf{r})|\mathbf{r}]$
and $H(\mathbf{s}|\mathbf{r})=-\log_{2}(P(\mathbf{s}|\mathbf{r}))$.\tabularnewline
\noalign{\vskip2pt}
$H(\mathbf{C}|\mathbf{w}\Vert\mathbf{r})$ & Cross entropy of $\mathbf{S}$ under $\mathbf{w}$ and $\mathbf{r}$
given by $\mathrm{E}_{\mathbf{C}}[H(\mathbf{s}|\mathbf{w})|\mathbf{r}]$.\tabularnewline
\noalign{\vskip2pt}
$\log_{2}(x)$ & Logarithm to the base $2$.\tabularnewline
\noalign{\vskip2pt}
$L_{i}(\mathbf{m})$ & Uncoded log. probability ratio given by $L_{i}(\mathbf{m})=r_{i}+w_{i}^{(1)}+w_{i}^{(2)}$.\tabularnewline
\noalign{\vskip2pt}
$L_{i}^{(a)}(\mathbf{r})$ & Overall log. ratio given by $L_{i}^{(a)}(\mathbf{r})=\frac{1}{2}\log_{2}\frac{P_{C_{i}}^{(a)}(+1|\mathbf{r})}{P_{C_{i}}^{(a)}(-1|\mathbf{r})}$.\tabularnewline
\noalign{\vskip2pt}
$L_{i}^{(l)}(\mathbf{m}^{(l)})$ & Constituent log. probability ratio obtained from $P_{C_{i}}^{(l)}(x|\mathbf{m}^{(l)})$.\tabularnewline
\noalign{\vskip2pt}
$L_{i}^{(l)}(\mathbf{m}^{(l)})$ & Extrinsic log. probability ratio of $P_{C_{i}}^{(l)}(x|\mathbf{m}^{(l)})\exp_{2}(-x(w_{i}^{(h)}-r_{i}))$
and $h\neq l$.\tabularnewline
\noalign{\vskip2pt}
$L_{i}^{\otimes}(\mathbf{m})$ & Common discriminated log. ratio of $P_{C_{i}}^{\otimes}(x|\mathbf{m})\propto\sum_{\mathbf{u}\in\mathbb{U}}\frac{P_{C_{i}}^{(1)}(x,\mathbf{u}|\mathbf{m}^{(1)})P_{C_{i}}^{(2)}(x,\mathbf{u}|\mathbf{m}^{(2)})}{P_{C_{i}}(x,\mathbf{u}|\mathbf{m})}$.\tabularnewline
\noalign{\vskip2pt}
$L_{i}^{{\scriptscriptstyle \boxtimes}}(\mathbf{m})$ & Distance log. ratio obtained from $P_{C_{i}}^{{\scriptscriptstyle \boxtimes}}(x|\mathbf{m})\propto\sum_{\mathbf{u}\in\mathbb{U}}\frac{P_{C_{i}}^{(1)}(\mathbf{u}|x,\mathbf{m}^{(1)})P_{C_{i}}^{(2)}(\mathbf{u}|x,\mathbf{m}^{(2)})}{P_{C_{i}}(\mathbf{u}|x,\mathbf{m})}$.\tabularnewline
\noalign{\vskip2pt}
$\mathbf{m}$ & Shorthand for $(\mathbf{r},\mathbf{w}^{(1)},\mathbf{w}^{(2)})$.\tabularnewline
\noalign{\vskip2pt}
$\mathbf{m}^{(l)}$ & Shorthand for $(\mathbf{r},\mathbf{w}^{(h)})$, $h\neq l$, and $h,l\in\{1,2\}$.\tabularnewline
\noalign{\vskip2pt}
$P^{(l)}(\mathbf{s}|\mathbf{m})$ & Shorthand for $P_{\mathbf{C}^{(l)}}(\mathbf{s}|\mathbf{m})$, the
probability of $\mathbf{s}$ under the $l$-th constituent code and
$\mathbf{m}$.\tabularnewline
\noalign{\vskip2pt}
$P(\mathbf{s}|\mathbf{r})$ & Probability $P_{\mathbf{S}|\mathbf{R}}(\mathbf{s}|\mathbf{r})$ of
$\mathbf{s}$ under $\mathbf{r}$.\tabularnewline
\noalign{\vskip2pt}
$P_{C_{i}}(x|\mathbf{r})$ & Probability of $S_{i}=C_{i}=x$ under $\mathbf{r}$.\tabularnewline
\noalign{\vskip2pt}
$P_{C_{i}}^{(c)}(x|\mathbf{r})$ & Probability of $C_{i}=x$ under $\mathbf{r}$ and the code restriction
$\mathbf{c}\in\mathbb{C}$; aka. $i$-th symbol belief.\tabularnewline
\noalign{\vskip2pt}
$\mathbf{r}$ & Received vector representing the channel information.\tabularnewline
\noalign{\vskip2pt}
$\mathbb{S}=\mathbb{E}(\mathbf{S})$ & Uncoded set given by all $\mathbf{s}=(s_{1},\ldots,s_{n})$ and $s_{i}\in\mathbb{B}$. \tabularnewline
\noalign{\vskip2pt}
$\tanh_{2}(x)$ & Tanh to the base $2$ given by $\frac{2^{x}-2^{-x}}{2^{x}+2^{-x}}$.\tabularnewline
\noalign{\vskip2pt}
$u_{l}$ & Correlation given by $u_{l}=\mathbf{s}\mathbf{w}^{(l)T}$.\tabularnewline
\noalign{\vskip2pt}
$\mathbb{U}=\mathbb{E}(\mathbf{U})$ & Set of possible discriminated or correlation values $\mathbf{u}=(u_{0},u_{1},u_{2})$.\tabularnewline
\noalign{\vskip2pt}
$\mathbf{w}^{(l)}$ & Transfer vector representing the beliefs of the $l$-th constituent
code, with $\mathbf{w}^{(0)}=\mathbf{r}$.\tabularnewline
\noalign{\vskip2pt}
$\mathbb{Z}_{2}$ & Integers $\mathbb{Z}$ mod $2$.\tabularnewline
\noalign{\vskip2pt}
\end{tabular}

